AbCD: A Component-wise Adjustable Framework for Dynamic Optimization Problems

Dynamic Optimization Problems (DOPs) are characterized by changes in the fitness landscape that can occur at any time and are common in real world applications. The main issues to be considered include detecting the change in the fitness landscape and reacting in accord. Over the years, several evolutionary algorithms have been proposed to take into account this characteristic during the optimization process. However, the number of available tools or open source codebases for these approaches is limited, making reproducibility and extensive experimentation difficult. To solve this, we developed a component-oriented framework for DOPs called Adjustable Components for Dynamic Problems (AbCD), inspired by similar works in the Multiobjective static domain. Using this framework, we investigate components that were proposed in several popular DOP algorithms. Our experiments show that the performance of these components depends on the problem and the selected components used in a configuration, which differs from the results reported in the literature. Using irace, we demonstrate how this framework can automatically generate DOP algorithm configurations that take into account the characteristics of the problem to be solved. Our results highlight existing problems in the DOP field that need to be addressed in the future development of algorithms and components.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> files/5-design.tex <==
\section{Design of Dynamic Evolutionary Algorithms}\label{design}

Here we show how to use AbCD to create new configurations of evolutionary algorithms for DOPs. We follow two different approaches: a manual design, where we select the components one by one, and an automatic design, where we use irace to find a well-performing configuration of the components altogether.

\subsection{Manual Design}

Assuming independence among the components, we do the manual configuration to select a configuration of the components and their parameterization that performances well in the problems, for each optimizer. First, we search for the best parameter in a wide range of values for each component independently. We start with the multipopulation, since some of the other components require more than one sub-population. Then we select one component and we search for its best parameterization. We repeat this process for each component. Finally, we combine these best configuration of components to create the $AbcD_{man}$. To evaluate performance, we use the offline error ($E_{o}$).

The nomenclature of the configuration generated by the framework is $AbCD_{ES{\%}}$, where $\%$ indicates the percentage of individuals in the population that uses ES as the optimizer, and the rest of the individuals use PSO. Thus, the $AbCD_{ES100}$ configuration indicates that 100\% of the individuals use the ES optimizer and the $AbCD_{ES0}$ configuration indicates that no individual use ES, that is, all are optimized by PSO. For all configuration explored, see Table \ref{abcd-algorithms}.

\input{files/tables/algorithms.tex}

% \subsubsection{Benchmark Problems}
To evaluate the components as well as test the generated algorithms, the Moving Peaks Benchmark (MPB) was used, as it is available from the Python library DEAP~\cite{DEAP_JMLR2012}. Among the predefined scenarios,we set MPB to the scenario 2, as it is frequently used~\cite{mQSO-2006, CPSO-2010, survey-phd-2011, FTMPSO-2013, GMPB-2022}.



\subsection{Automatic Design}
Assuming dependence among the components, we use irace~\cite{LOPEZIBANEZ201643} to automatically design an $AbCD_{auto}$ configuration based on the components available in our framework. We run irace with its default settings, except for the number of elite configurations tested, which we increase from 1 to 7, following Campelo et al. work~\cite{moeadr_paper}. We run irace with a budget of $30 000$ runs. In a preliminary run of irace, we found that we were facing a heterogeneous scenario, and thus adjusted the configuration and increased the number of instances executed before doing a statistical test to $10$, the number of instances evaluated between elimination tests to $5$, and increase the number of new instances executed in each iteration to $5$ as recommended in irace's user guide\footnote{https://mlopez-ibanez.github.io/irace/irace-package.pdf, accessed 17th January 2023} and by Souza et al.~\cite{DESOUZA2021100186}. Here, we use the offline error ($E_{o}$) as the training metric for evaluating the instances generated automatically by irace. We chose to fix the parameter $\chi = 1$ to reduce the number of parameters of PSO and the range of $\phi_1$ and $\phi_2$ was based on the work of Camacho-Villalón et al.\cite{pso-automated-2022}. Finally, each configuration runs for $500000$ evaluations.

% \subsubsection{Training and testing}

We use the same set of the MPB as in the manual design. Since we aim to find good configurations to perform well in many problems, we use more instances than those used in the manual design. These instances show vary not only the positions of the optimal points change but also the dimensions and the number of peaks. 

% In order to bring the problem closer to a real world problem, where not infrequently, not only the positions of the optimal points change but also the dimensions and the number of individuals can change, we will set irace to train and test in more than one scenario, and the parameters will be chosen taking into account all scenarios. The idea is to obtain an algorithm that is capable of performing well not only in one scenario but also versatile.


==> files/components/algo.tex <==
\begin{algorithm}[htbp]
	\caption{AbCD framework}\label{algo:abcd}
	\begin{algorithmic}[1]
        \State Get a configuration
		\State Initialize and evaluate the initial population $pop$
		\State Initialize the control list $restart$ with $False$ and size equal to the number of subpopulations $N_{subpops}$.\label{not-restart-0}
        \State Initialize the individual type list $ES_{ind}$ with percentage of $ES$ individuals in $pop$ \label{ES-individuals}
        \State $P_{best} \gets best$  of $pop$
        \State update($pop$)
        \If{Multipopulation is True}
            \State $pop$ = Multipopulation($pop$) \Comment{(G)}\label{multipopulation-1}
        \EndIf
		\While{\textit{Number of fitness evaluations is not reached}}
            % \State Initialize an empty control list $randomizeList$
            \If{Multipopulation is True}
                \If{Exclusion is True}
                    \State $restart$ = exclusion($pop$) \Comment{(G)}\label{randomizeList-1}
                \EndIf
                \If{Anti-Convergence is True}
                    \State $restart$ = antiConvergence($pop$) \Comment{(L)}\label{randomizeList-2}
                \EndIf
            \EndIf
            \If{Local-Search is True}
                \State $P_{best}$ = localSearch($P_{best}$) \Comment{(G)}
            \EndIf           
		    \For{\textbf{each} subpopulation $subpop$ in $pop$}
                \State $restart$ = reevaluate($subpop$)\label{not-randomizeList} \Comment{Change detection}
                \If{$subpop$ in $restart$} \Comment{(Lines~\ref{randomizeList-1},~\ref{randomizeList-2})}
                        \State randomize($subpop$)
                \Else \Comment{sub.pop not in $restart$ (Lines \ref{not-restart-0} or \ref{not-randomizeList})}
                    \For{\textbf{each} individual $i$ in $subpop$}
                        \If{$i$ in $ES_{ind}$ }
                            \State $i$ = ES($i$, $subpop$) %\Comment{Add the required pars.}
                        \Else
                            \State $i$ = PSO($i$, $subpop$) %\Comment{Add the required pars.}
                        \EndIf
                        \State update($pop$)
                    \EndFor
                \EndIf
                
            \EndFor
		\EndWhile
	\end{algorithmic}
\end{algorithm}

==> files/components/anti-convergence.tex <==
\begin{algorithm}[htbp]
	\caption{Anti-convergence}\label{algo:anti-convergence}
	\begin{algorithmic}[1]
        \Require population $pop$ and control list $restart$
        \State $converged \gets True$
        \State $S_{best_{worst.sub}} \gets Inf$ \Comment{Highest fitness value for an individual}
        \For{\textbf{each} subpopulation $subpop$ in $pop$}
            \State $S_{best} \gets$ best of $subpop$
                % \For{\textbf{each pair} $i_{j}, i_{k}$ in  $sub.pop$}   
                \For{\textbf{each} pair of individuals in  $subpop$}   
                    \State $distance$ = Euclidean distance per dimension
                    \State $max.dist$ = Get the maximum value of $distance$
                    \If {$max.dist$ > $r_{conv}$}
                        \State $converged \gets False$  \Comment{The $subpop$ didn't converge}\label{not-converged-line}
                    \EndIf
                    
                \EndFor
            \If{$f(S_{best_{worst.sub}}) < f(S_{best_{subpop}})$}
                \State $S_{best_{worst.sub}} \gets S_{best_{subpop}}$
            \EndIf
        \EndFor
        \If{$converged \ is \ True$} \Comment{All $subpops$ converged}
            \State $restart[S_{best_{worst.sub}}] \gets True$ \Comment{Restart the worst}
        \EndIf
        \State \textbf{Return} $restart$
	\end{algorithmic}
\end{algorithm}

==> files/components/es.tex <==
\begin{algorithm}[htbp]
	\caption{ES}\label{algo:es}
	\begin{algorithmic}[1]
        \Require Individual $i$ and its subpopulation $subpop$
        \State $S_{best} \gets best$  of $subpop$
        \For {\textbf{each} dimension $d$ in $i$}
            % \State $x_{i}^{d} = x_{S_{best}}^{d} + rand[0,1]r_{cloud}$
            \State $x_{i}^{d}$ = Equation\ref{es-posi}($d$, $S_{best}$)
            % \State u $\gets$ $rand()$ 
            % \State $x = x_{best_{sub.pop}} + u*r_{cloud} $\Comment{Eq.~\ref{es-posi}}
        \EndFor
        \State \textbf{Return} $i$
	\end{algorithmic}
\end{algorithm}




==> files/components/exclusion.tex <==
\begin{algorithm}[htbp]
	\caption{Exclusion}\label{algo:exclusion}
	\begin{algorithmic}[1]
        \Require population $pop$ and control list $restart$
        \For{\textbf{each pair of} subpopulations $subpop_1$, $subpop_2$ in $pop$}
            % \If{$s_1$ and $s_2$ not in $randomizeList[:]$}
                \State $distance$ $\gets$ euclideanDistance($S_{best_{subpop_{1}}}$,  $S_{best_{subpop_{2}}}$)
                \If{$distance < r_{excl}$}
                    \If{f($S_{best_{subpop_{1}}}$) < f($S_{best_{subpop_{2}}}$)}
                        \State $restart[subpop_1] \gets$ True
                    \Else
                        \State $restart[subpop_2] \gets$ True
                    \EndIf
                \EndIf
        \EndFor
        \State \textbf{Return} $restart$
	\end{algorithmic}
\end{algorithm}

==> files/components/local-search.tex <==
\begin{algorithm}[htbp]
	\caption{Local Search}\label{algo:local-search}
	\begin{algorithmic}[1]
        \Require individual $P_{best}$
        \For  {1 to $etry$}
            \State $P_{best}^{'} \gets P_{best}$ 
            \For{\textbf{each} dimension $d$ in $P_{best}^{'}$}
                % \State u $\gets$ $rand()$ 
                % \State $new = best + u*r_{cloud} $\Comment{Eq.~\ref{ls-posi}}
                \State $x_{P_{best}}^{'d}$ = Equation\ref{ls-posi}($P_{best}^{'}$)
            \EndFor
        \If {$f(P_{best}) < f(P_{best}^{'})$}
            \State $f(P_{best}) \gets f(P_{best}^{'})$
        \EndIf
        \EndFor
        \State \textbf{Return} $P_{best}$
	\end{algorithmic}
\end{algorithm}

==> files/components/multipopulation.tex <==
\begin{algorithm}[htbp]
	\caption{Multi-population}\label{algo:multipopulation}
	\begin{algorithmic}[1]
        \Require population $pop$
        \State $pop^{'} \gets$ list of $N_{subpops}$ size
        \For{\textbf{each} subpopulation $subpop$ in $pop^{'}$}
            \State $subpop \gets pop/N_{subpops}$ 
        \EndFor
        \State \textbf{Return} $pop^{'}$
	\end{algorithmic}
\end{algorithm}

==> files/components/pso.tex <==
\begin{algorithm}[htbp]
	\caption{PSO}\label{algo:pso}
	\begin{algorithmic}[1]
        \Require Individual $i$ and its subpopulation $subpop$
        \State $S_{best}$ $\gets$ best of $subpop$
        \For{\textbf{each} dimension $d$ in $i$}
            \State $v_{i}^{d}$ = Equation\ref{pso-velo}($i$, $d$, $S_{best}$)
        \EndFor
        \State $\vec{x}_{i}$ = Equation\ref{pso-posi}($i$, $\vec{v}_{i}$)
        \State \textbf{Return} $i$
	\end{algorithmic}
\end{algorithm}

==> files/components/reevaluation.tex <==
\begin{algorithm}[htbp]
	\caption{Reevaluate $S_{best}$}\label{algo:reevaluation}
	\begin{algorithmic}[1]
        \Require subpopulation $subpop$ and control list $restart$
        \State $S_{best} \gets$ best of $subpop$
        \State sensor $\gets$ evaluate($S_{best}$)
        \If{$sensor \ != f(S_{best})$} \Comment{If different, a change occurred}
            \State evaluate($subpop$) \Comment{Reevaluate the entire subpopulation}
            \State $restart[subpop] \gets False$
        \EndIf
        \State \textbf{Return} \textit{restart}
	\end{algorithmic}
\end{algorithm}

==> files/tables/algorithms.tex <==
\begin{table}[htbp]
\centering
	\scriptsize
	%\caption{AbCD optimizers}
    \caption{AbCD optimizers and the percentage of solutions in a population following PSO or ES.}
	\label{abcd-algorithms}
    \begin{tabular}{c|c|c}
        % \hline
        \rowcolor[gray]{.85} Optimizers      & PSO Individuals & ES Individuals           \\ 
        \multirow{1}{*}{$PSO (AbCD_{ES0})$}   & $100\%$ & $0\%$    \\ \hline     
        \multirow{1}{*}{$AbCD_{ES25} $}   & $75\%$ & $25\%$    \\ \hline     
        \multirow{1}{*}{$AbCD_{ES50} $}   & $50\%$ & $50\%$    \\ \hline     
        \multirow{1}{*}{$AbCD_{ES75} $}   & $25\%$ & $75\%$    \\ \hline     
        \multirow{1}{*}{$ES (AbCD_{ES100})$}   & $0\%$ & $100\%$    \\   
        \end{tabular}
        % \vspace{-1.5em}
\end{table}


==> files/tables/configurations.tex <==
\begin{table*}[htbp]
\centering
    \scriptsize
	%\footnotesize
	\caption{Configurations generated with AbCD framework}
	\label{configurations}
    \begin{tabular}{l|c|c|c|c}
        \rowcolor[gray]{.85} Optimizer & Multipopulation & Exclusion & Local search & Anti-Convergence \\ \hline
        
        \begin{tabular}{l}  
                            PSO $\rightarrow$ $\begin{cases} \chi = 0.729, \phi_1 = 2.05, \phi_2 = 2.05 \end{cases}$
                            \end{tabular} & Disabled & Disabled & Disabled & Disabled  \\ \hline
        \begin{tabular}{l}
                            ES $\rightarrow$ $\begin{cases} r_{cloud} = 0.05 \end{cases}$
                            \end{tabular} & Disabled & Disabled & Disabled & Disabled \\ \hline
        \begin{tabular}{l}
                            mQSO~\cite{mQSO-2006}$\rightarrow$ $\begin{cases} \chi = 0.729, \phi_1 = 2.05, \phi_2 = 2.05 \\ r_{cloud} = 1  \\ \end{cases}$
                            \end{tabular} & $N_{subpop}=10$ & $r_{excl} = 22.9$ & Disabled & $r_{conv} = 39.7$ \\ \hline
        \begin{tabular}{l}  
                            $AbCD_{man}$ $\rightarrow$ $\begin{cases} \% = 75,r_{cloud} = 0.05 \\ \chi=0.729, \phi_1 = 2.05, \phi_2 = 2.05 \\  \end{cases}$
                            \end{tabular} & Disabled & Disabled & Disabled & Disabled  \\ \hline
        \begin{tabular}{l}  
                            $AbCD_{auto}$ $\rightarrow$ $\begin{cases} \% = 75, r_{cloud} = 0.2 \\ \chi=1, \phi_1 = 1.38, \phi_2 = 2.24 \\   \end{cases}$
                            \end{tabular} & $N_{subpop}=25$ & Disabled & $\begin{cases} r_{ls} = 2.9 \\ etry = 2 \end{cases}$  &  Disabled \\ 
                   
        \end{tabular}
\end{table*}



==> files/tables/pso-es.tex <==
\begin{table}[htbp]
\centering
	%\small
    \scriptsize
	\caption{Standard PSO and ES from AbCD framework on MPB}
	\label{pso-es-results}
    \begin{tabular}{l|l|l}
        % \hline   
        \rowcolor[gray]{.85}Optimizer & Parameters & Results \\ \hline
        \multirow{1}{*}{PSO} & \begin{tabular}{l} $\begin{cases} \phi_1 = 1.4962 \\ \phi_2 = 1.4962 \end{cases}$ \end{tabular} & \begin{tabular}{@{}c@{}}$ E_{o} = 21.3409(1.2851)$ \\ $E_{b} = $ \\ $A_{rr} = $ \end{tabular} \\ \hline  
        \multirow{1}{*}{ES} & $r_{cloud} = 1$ & \begin{tabular}{@{}c@{}}$ E_{o} = 25.6913(0.5894)$ \\ $E_{b} = $ \\ $A_{rr} = $ \end{tabular} \\ %\hline  
        \end{tabular}
\end{table}


==> files/tables/results-manual-parameters.tex <==
\begin{table}[htpb]
\centering
	\scriptsize 
	% \caption{Standard PSO and ES from AbCD framework on MPB}
	\caption{Parameters values with the best performance individually in each optimizer.}
    \label{results-manual-parameters}
    \scriptsize
     \begin{tabular}{l|l|l|l|l}
         %\hline   
         \rowcolor[gray]{.85}Optimizer &  parameters & $E_{o}$ & $E_{b}$ & $A_{rr}$  \\
         {\begin{tabular}{@{}c@{}} PSO \end{tabular}} & \begin{tabular}{@{}c@{}}$ r_{excl} = 0$ \\ $r_{conv} = 0.5 $ \\ $r_{ls} = 0$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 20.1826(1.3809)$ \\ $20.1817(1.3828)$ \\ $20.1826(1.3809)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 17.9729(1.5292)$ \\ $17.9717(1.5292)$ \\ $17.9729(1.5292)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 22.0283(0.2219)$ \\ $21.4933(1.2050)$ \\ $21.3409(1.2851)$ \end{tabular} \\ \hline
         
        {$AbCD_{ES25}$} & \begin{tabular}{@{}c@{}}$ r_{excl} = 0$ \\ $r_{conv} = 0 $ \\ $r_{ls} = 0 $ \end{tabular} & \begin{tabular}{@{}c@{}}$ 19.7556(1.2184)$ \\ $19.7556(1.2184)$ \\ $19.7556(1.2184)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 17.8491(1.3721)$ \\ $17.8491(1.3721)$ \\ $17.8491(1.3721)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 22.0283(0.2219)$ \\ $21.4933(1.2050)$ \\ $21.3409(1.2851)$ \end{tabular} \\ \hline

         {\hl{$AbCD_{ES50}$}} & \begin{tabular}{@{}c@{}}$ r_{excl} = 0$ \\ \hl{$r_{conv} = 0.5 $} \\ $r_{ls} = 0 $ \end{tabular} & \begin{tabular}{@{}c@{}}$ 19.5932(1.1950)$ \\ \hl{$19.4507(1.4969)$} \\ $19.5932(1.1950)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 17.8498(1.3774)$ \\ $17.6387(1.7510)$ \\ $17.8498(1.3774)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 22.0283(0.2219)$ \\ $21.4933(1.2050)$ \\ $21.3409(1.2851)$ \end{tabular} \\ \hline
         
         {$AbCD_{ES75}$} & \begin{tabular}{@{}c@{}} $ r_{excl} = 0$ \\ $r_{conv} = 0.5 $ \\ $r_{ls} = 0 $ \end{tabular} & \begin{tabular}{@{}c@{}}$ 19.5737(1.3541)$ \\ $19.5525(1.4931)$ \\ $19.5737(1.3541)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 17.8654(1.5834)$ \\ $17.7980(1.7404)$ \\ $17.8654(1.5834$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 22.0283(0.2219)$ \\ $21.4933(1.2050)$ \\ $21.3409(1.2851)$ \end{tabular} \\ \hline
         
         {\begin{tabular}{@{}c@{}} ES \end{tabular}} & \begin{tabular}{@{}c@{}}$ r_{excl} = 40$ \\ $r_{conv} = 0.5 $ \\ $r_{ls} = 2$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 23.9425(2.1406)$ \\ $21.1875(1.7461)$ \\ $23.3576(2.2976)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 17.6190(2.2365)$ \\ $16.8021(1.8355)$ \\ $16.1188(2.5955)$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 22.0283(0.2219)$ \\ $21.4933(1.2050)$ \\ $21.3409(1.2851)$ \end{tabular} \\ %\hline  
         \end{tabular}
\end{table}


==> files/tables/scenarios-results.tex <==
\begin{table}[htbp]
\centering
    \scriptsize
	%\footnotesize
	\caption{$E_{o}$ and $E_{b}$ results of the different configurations}
	\label{manual-resulsts}
    \begin{tabular}{c|c|c|c|c|c}
        \rowcolor[gray]{.85}Algorithm & 5D-10P-1s & 8D-8P-1s & 8D-10P-1s & 10D-8P-1s & 10D-10P-1s \\ \hline
        
        $PSO$ & 
                            \begin{tabular}{l} $E_{o} = 15.1205(1.6212)$ \\ $E_{b} = 12.0082(1.2456)$ \\ %$A_{rr} =  $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 12.5545(0.4421)$ \\ $E_{b} = 12.6071(0.5472)$ \\ %$A_{rr} = 0.1991(0.2307)$ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 13.0074(2.4277)$ \\ $E_{b} = 10.9352(2.4355)$ \\ %$A_{rr} = 0.1619(0.1842) $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 9.7193(0.0350)$ \\ $E_{b} = 7.0681(0.1585)$ \\ %$A_{rr} = 0.1235(0.0049)$ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 19.4187(0.0248)$ \\ $E_{b} = 17.6928(0.2105)$ \\ %$A_{rr} = 0.1922(0.0050)$ \\  
                            \end{tabular} \\ \hline
        $ES$ & 
                            \begin{tabular}{l} $E_{o} = 14.6344(1.7055)$ \\ $E_{b} = 12.5183(1.3381)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 12.2455(0.1653)$ \\ $E_{b} = 12.6244(0.7111)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 13.1655(2.7125)$ \\ $E_{b} = 11.6927(2.8395)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 9.5437(0.1560)$ \\ $E_{b} = 7.2762(0.0643)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 19.0403(0.1172)$ \\ $E_{b} = 17.9531(0.1840)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} \\ \hline
        $mQSO$\cite{mQSO-2006} & 
                            \begin{tabular}{l} $E_{o} = 7.9720(1.2126)$ \\ $E_{b} = 5.3081(1.3536)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 12.8583(1.4839)$ \\ $E_{b} = 10.3264(1.6611)  $ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 13.64423(0.6601)$ \\ $E_{b} = 11.8551(0.9271)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 12.8789(0.6371)$ \\ $E_{b} = 10.6514(0.7802) $ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 23.3567(0.8941)$ \\ $E_{b} = 20.7601(0.9761) $ \\ %$A_{rr} = $ \\  
                            \end{tabular} \\ \hline
        $AbCD_{man}$ & 
                            \begin{tabular}{l} $E_{o} = 14.7765(1.7097)$ \\ $E_{b} = 12.5147(1.3629)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 12.0514(0.0737)$ \\ $E_{b} = 12.4550(0.4910)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 12.8008(2.5273)$ \\ $E_{b} = 11.4130(2.6814)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} \hl{$E_{o} = 9.1701(0.0388)$} \\ $E_{b} = 7.1212(0.1329)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} \hl{$E_{o} = 18.7176(0.0320)$} \\ $E_{b} = 17.7534 (0.2473) $ \\ %$A_{rr} = $ \\  
                            \end{tabular} \\ \hline
        $AbCD_{auto}$ & 
                            \begin{tabular}{l} \hl{$E_{o} = 6.3743(0.7052)$} \\ $E_{b} = 3.7441(0.8709)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} \hl{$E_{o} = 8.0995(1.8802)$} \\ $E_{b} = 5.6423(2.2541)$ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} \hl{$E_{o} = 11.10450(1.2338)$} \\ $E_{b} = 9.4679(1.5722) $ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 10.9760(1.2956)$ \\ $E_{b} = 9.2836(1.6564) $ \\ %$A_{rr} = $ \\  
                            \end{tabular} & 
                            \begin{tabular}{l} $E_{o} = 19.9026(2.4871)$ \\ $E_{b} = 18.0199(2.9705)$ \\ %$A_{rr} = $ \\
                            \end{tabular} \\                                            
        \end{tabular}
\end{table}




==> files/tables/subpop.tex <==
% \begin{table*}[htbp]
% \centering
% 	 \small
% 	% \caption{Standard PSO and ES from AbCD framework on MPB}
% 	\caption{Offline error of optimizers varying the number of subpopulations $N_{subpops}$, with $r_{cloud}=0.05$}
% 	\label{subpopulations-table}
%      \begin{tabular}{l|l|l}
%          % \hline   
%          \rowcolor[gray]{.85}Optimizer & Multi-population & Offline Error \\ \hline
%          \multirow{1}{*}{$AbCD_{ES0}(PSO)$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 19.4187(0.0248)$ \\ $20.0468(0.0287)$ \\ $20.1826(1.3809)$ \\ $25.2869(2.0204)$ \\ $33.9557(3.7422)$ \\ $99.2788(20.6676)$ \\ $157.3536(11.8929)$ \end{tabular} \\ \hline
%          {$AbCD_{ES25}$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}} $18.8832(0.0186)$ \\ $19.6459(0.0236)$ \\ $19.7556(1.2184)$ \\ $19.5041(2.1427)$ \\ $19.5660(2.4690)$ \\ $99.2788(20.6676)$ \\ $157.3536(11.8929)$ \end{tabular} \\ \hline
%          {$AbCD_{ES50}$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}} $18.7498(0.0232)$ \\ $19.4912(0.281)$ \\ $19.5932(1.1950)$ \\ $19.5563(2.1798)$ \\ $19.8819(2.4329)$ \\ $66.7334(12.2673)$ \\ $157.3536(11.8929)$ \end{tabular} \\ \hline
%          {$AbCD_{ES75}$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}}$18.7176(0.0320)$ \\ $19.2591(0.9935)$ \\ $19.5737(1.3541)$ \\ $19.9342(2.1658)$ \\ $24.4162(1.9479)$ \\ $66.7334(12.2673)$ \\ $157.3536(11.8929)$ \end{tabular} \\ \hline
%          {$AbCD_{ES100}(ES)$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}} $19.0403(0.1172)$ \\ $22.06689(1.0232)$ \\ $24.5242(2.5880)$ \\ $41.5702(4.6395)$ \\ $54.6549(9.3672)$ \\ $107.9224(20.7775)$ \\ $140.0417(12.0578)$ \end{tabular} \\
%          \end{tabular}
% \end{table*}

% \begin{table*}[htbp]
% \centering
% 	 \small
% 	% \caption{Standard PSO and ES from AbCD framework on MPB}
% 	\caption{Offline error of optimizers varying the number of subpopulations $N_{subpops}$, with $r_{cloud}=0.05$}
% 	\label{subpopulations-table}
%      \begin{tabular}{l|l|l}
%          % \hline   
%          \rowcolor[gray]{.85}Optimizer & Multi-population & Offline Error \\ \hline
%          \multirow{1}{*}{$PSO (AbCD_{ES0})$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}}$ 19.4187(0.0248)$ \\ $20.0468(0.0287)$ \\ $20.1826(1.3809)$ \\ $25.2869(2.0204)$ \\ $33.9557(3.7422)$ \\ $99.2788(20.6676)$ \\ $157.3536(11.8929)$ \end{tabular} \\ \hline
%          {$AbCD_{ES25}$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}} $18.8832(0.0186)$ \\ $19.6459(0.0236)$ \\ $19.7556(1.2184)$ \\ $19.5041(2.1427)$ \\ $19.5660(2.4690)$ \\ $99.2788(20.6676)$ \\ $157.3536(11.8929)$ \end{tabular} \\ \hline
%          {$AbCD_{ES50}$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}} $18.7498(0.0232)$ \\ $19.4912(0.281)$ \\ $19.5932(1.1950)$ \\ $19.5563(2.1798)$ \\ $19.8819(2.4329)$ \\ $66.7334(12.2673)$ \\ $157.3536(11.8929)$ \end{tabular} \\ \hline
%          {$AbCD_{ES75}$} & \begin{tabular}{@{}c@{}} $N_{subpops} = 1$ \\ $N_{subpops} = 5$ \\ $N_{subpops} = 10$ \\ $N_{subpops} = 20$ \\ $N_{subpops} = 25$ \\ $N_{subpops} = 50$ \\ $N_{subpops} = 100$ \end{tabular} & \begin{tabular}{@{}c@{}}$18.7176(0.0320)$ \\ $19.2591(0.9935)$ \\ $19.5737(1.3541)$ \\ $19.9342(2.1658)$ \\ $24.4162(1.9479)$ \\ $66.7334(12.2673)$ \\ $157.3536(11.8929)$ \end{tabular} \\ \hline
\begin{table*}[htbp]
\centering
	 %\small
  \scriptsize
	% \caption{Standard PSO and ES from AbCD framework on MPB}
	\caption{Offline error (and standard deviation) of optimizers varying the number of subpopulations $N_{subpops}$, with $r_{cloud}=0.05$}
	\label{subpopulations-table}
     \begin{tabular}{c|c|c|c|c|c}
         % \hline   
         \rowcolor[gray]{.85} $N_{subpops}$ & PSO & $AbCD_{ES25}$ & $AbCD_{ES50}$ & $AbCD_{ES75}$ & ES \\ \hline
         1 & $19.4187(0.0248)$ & $18.8832(0.0186)$ & $18.7498(0.0232)$ & $18.7176(0.0320)$ & $19.0403(0.1172)$ \\ \hline
        5  & $20.0468(0.0287)$ & $19.6459(0.0236)$ & $19.4912(0.281)$  & $19.2591(0.9935)$ & $22.06689(1.0232)$ \\ \hline
        10  & $20.1826(1.3809)$ & $19.7556(1.2184)$ & $19.5932(1.1950)$  & $19.5737(1.3541)$ & $24.5242(2.5880)$ \\ \hline
        20  & $25.2869(2.0204)$ & $19.5041(2.1427)$ & $19.5563(2.1798)$  & $19.9342(2.1658)$ & $41.5702(4.6395)$ \\ \hline
        25  & $33.9557(3.7422)$ & $19.5660(2.4690)$ & $19.8819(2.4329)$  & $24.4162(1.9479)$ & $54.6549(9.3672)$ \\ 
         \end{tabular}
\end{table*}

